Enhancements in cross-temporal forecast reconciliation, with an application to solar irradiance forecasts

In recent works by Yang et al. (2017a,b), and Yagli et al. (2019), geographical, temporal, and sequential deterministic reconciliation of hierarchical photovoltaic (PV) power generation have been considered for a simulated PV dataset in California. In the first two cases, the reconciliations are carried out in spatial and temporal domains separately. To further improve forecasting accuracy, in the third case these two reconciliation approaches are sequentially applied. During the replication of the forecasting experiment, some issues emerged about non-negativity and coherence (in space and/or in time) of the sequentially reconciled forecasts. Furthermore, while the accuracy improvement of the considered approaches over the benchmark persistence forecasts is clearly visible at any data granularity, we argue that an even better performance may be obtained by a thorough exploitation of cross-temporal hierarchies. In this paper the cross-temporal point forecast reconciliation approach is applied to generate non-negative, fully coherent (both in space and time) forecasts. In particular, some relationships between two-step, iterative and simultaneous cross-temporal reconciliation procedures are for the first time established, non-negativity issues of the final reconciled forecasts are correctly dealt with in a simple way, and the most recent cross-temporal reconciliation approaches are adopted. The normalised Root Mean Square Error is used to measure forecasting accuracy, and a statistical multiple comparison procedure is performed to rank the approaches. Besides assuring full coherence, and non-negativity of the reconciled forecasts, the results show that for the considered dataset, cross-temporal forecast reconciliation significantly improves on the sequential procedures proposed by Yagli et al. (2019), at any cross-sectional level of the hierarchy and for any temporal granularity.

==> preamble/mathdef.tex <==
% \widebreve{}
\makeatletter
\def\widebreve{\mathpalette\wide@breve}
\def\wide@breve#1#2{\sbox\z@{$#1#2$}%
	\mathop{\vbox{\m@th\ialign{##\crcr
				\kern0.08em\brevefill#1{0.8\wd\z@}\crcr\noalign{\nointerlineskip}%
				$\hss#1#2\hss$\crcr}}}\limits}
\def\brevefill#1#2{$\m@th\sbox\tw@{$#1($}%
	\hss\resizebox{#2}{\wd\tw@}{\rotatebox[origin=c]{90}{\upshape(}}\hss$}
%\makeatletter
\makeatother

% \widecheck{}
\makeatletter
\DeclareRobustCommand\widecheck[1]{{\mathpalette\@widecheck{#1}}}
\def\@widecheck#1#2{%
	\setbox\z@\hbox{\m@th$#1#2$}%
	\setbox\tw@\hbox{\m@th$#1%
		\widehat{%
			\vrule\@width\z@\@height\ht\z@
			\vrule\@height\z@\@width\wd\z@}$}%
	\dp\tw@-\ht\z@
	\@tempdima\ht\z@ \advance\@tempdima2\ht\tw@ \divide\@tempdima\thr@@
	\setbox\tw@\hbox{%
		\raise\@tempdima\hbox{\scalebox{1}[-1]{\lower\@tempdima\box
				\tw@}}}%
	{\ooalign{\box\tw@ \cr \box\z@}}}
\makeatother

%daniele
\usepackage{array}
\usepackage{scalerel,stackengine}
\stackMath
\newcommand\reallywidehat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern-.6pt\bigwedge\kern-.6pt}%
    {\rule[-\textheight/2]{1ex}{\textheight}}%WIDTH-LIMITED BIG WEDGE
  }{\textheight}% 
}{0.5ex}}%
\stackon[1pt]{#1}{\tmpbox}%
}

\newcommand\norm[1]{\left\lVert#1\right\rVert}

%\newcommand{\1vet}{\textbf{1}}
\newcommand{\alphavet}{\pmb{\alpha}}
\newcommand{\betavet}{\pmb{\beta}}
\newcommand{\etavet}{\pmb{\eta}}
\newcommand{\epsvet}{\pmb{\varepsilon}}
\newcommand{\lambdavet}{\pmb{\lambda}}
\newcommand{\avet}{\textbf{a}}
\newcommand{\bvet}{\textbf{b}}
\newcommand{\cvet}{\textbf{c}}
\newcommand{\dvet}{\textbf{d}}
\newcommand{\evet}{\textbf{e}}
\newcommand{\fvet}{\textbf{f}}
\newcommand{\gvet}{\textbf{g}}
\newcommand{\lvet}{\textbf{l}}
\newcommand{\pvet}{\textbf{p}}
\newcommand{\qvet}{\textbf{q}}
\newcommand{\rvet}{\textbf{r}}
\newcommand{\svet}{\textbf{s}}
\newcommand{\tvet}{\textbf{t}}
\newcommand{\uvet}{\textbf{u}}
\newcommand{\vvet}{\textbf{v}}
\newcommand{\wvet}{\textbf{w}}
\newcommand{\xvet}{\textbf{x}}
\newcommand{\yvet}{\textbf{y}}
\newcommand{\zvet}{\textbf{z}}
\newcommand{\Avet}{\textbf{A}}
\newcommand{\Bvet}{\textbf{B}}
\newcommand{\Cvet}{\textbf{C}}
\newcommand{\Dvet}{\textbf{D}}
\newcommand{\Evet}{\textbf{E}}
\newcommand{\Fvet}{\textbf{F}}
\newcommand{\Gvet}{\textbf{G}}
\newcommand{\Hvet}{\textbf{H}}
\newcommand{\Ivet}{\textbf{I}}
\newcommand{\Jvet}{\textbf{J}}
\newcommand{\Kvet}{\textbf{K}}
\newcommand{\Lvet}{\textbf{L}}
\newcommand{\Mvet}{\textbf{M}}
\newcommand{\Nvet}{\textbf{N}}
\newcommand{\Pvet}{\textbf{P}}
\newcommand{\Qvet}{\textbf{Q}}
\newcommand{\Rvet}{\textbf{R}}
\newcommand{\Svet}{\textbf{S}}
\newcommand{\Tvet}{\textbf{T}}
\newcommand{\Uvet}{\textbf{U}}
\newcommand{\Wvet}{\textbf{W}}
\newcommand{\Xvet}{\textbf{X}}
\newcommand{\Yvet}{\textbf{Y}}
\newcommand{\Zvet}{\textbf{Z}}
\newcommand{\Zerovet}{\textbf{0}}
%\bmdefine{\ahvet}{\mathsf{a}}
%\bmdefine{\bhvet}{\mathsf{b}}
\bmdefine{\xhvet}{\mathsf{x}}
\bmdefine{\yhvet}{\mathsf{y}}
\bmdefine{\Chvet}{\mathsf{C}}
\bmdefine{\Ghvet}{\mathsf{G}}
\bmdefine{\Jhvet}{\mathsf{J}}
\bmdefine{\Shvet}{\mathsf{S}}
\bmdefine{\Uhvet}{\mathsf{U}}
\bmdefine{\Gammavet}{\mathsf{\Gamma}}
\bmdefine{\Omegavet}{\mathsf{\Omega}}
\bmdefine{\Sigmavet}{\mathsf{\Sigma}}
\bmdefine{\Thetavet}{\mathsf{\Theta}}
\bmdefine{\ahvet}{\mathfrak{a}}
\bmdefine{\bhvet}{\mathfrak{b}}
%\bmdefine{\xhvet}{\mathfrak{x}}
%\bmdefine{\yhvet}{\mathfrak{y}}
%\bmdefine{\Chvet}{\mathfrak{C}}
%\bmdefine{\Ghvet}{\mathfrak{G}}
%\bmdefine{\Jhvet}{\mathfrak{J}}
%\bmdefine{\Shvet}{\mathfrak{S}}
%\bmdefine{\Uhvet}{\mathfrak{U}}

%\newcommand{\ahvet}{{\bm{\mathsf{a}}}
%\newcommand{\bhvet}{{\bm{\mathsf{b}}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

==> tab/appTDF_DG_PV324.tex <==
%\newpage
\section{Proof of the theorem}

	\begin{enumerate}
		\item Let $\Uvet'_{n_a \times n}$  and $\Zvet'_{m \times (k^\ast + m)}$ be the cross-sectional and temporal, respectively, zero constraints kernel matrix. Let
		$$
		\Mvet_{cs}^{[k]} = \Mvet_{cs} = \left[\Ivet_n - \Wvet\Uvet\left(\Uvet'\Wvet\Uvet\right)^{-1}\Uvet'\right], \quad k \in \mathcal{K}
		$$
		and
		$$
		\Mvet_{te,i} = \Mvet_{te} = \left[\Ivet_{k^\ast+m} - \Omegavet\Zvet\left(\Zvet'\Omegavet\Zvet\right)^{-1}\Zvet'\right], \quad i=1,\ldots,n ,
		$$
		be the cross-sectional and temporal projection matrices, respectively, such that:
		$$
		\begin{array}{rcll}
			\widetilde{\Yvet}_{cs}^{[k]} & = & \Mvet_{cs}\widehat{\Yvet}^{[k]}, & k \in \mathcal{K}, \\
			\widetilde{\yvet}_{te,i}      & = & \Mvet_{te}\widehat{\yvet}_i,      & i=1,\ldots,n,
		\end{array}
		$$
		where
%		\begin{itemize}
%			\item
$\widehat{\Yvet}^{[k]}$ and $\widetilde{\Yvet}_{cs}^{[k]}$ are the $\left( n \times \frac{m}{k}\right)$ matrices with, respectively, the base and the cross-sectional reconciled forecasts of the $n$ series at time granularity $k$, and
			%\item
			 $\widehat{\yvet}_i$ and $\widetilde{\yvet}_{t,i}$ are the $\left[ (k^*+m) \times 1\right]$ vectors with, respectively, the base and the temporal reconciled forecasts at all time granularities for the $i$-th series.
%		\end{itemize}
		In compact matrix form we get:
		$$
		\begin{array}{rcl}
			\widetilde{\Yvet}_{cs} & = & \left[ \widetilde{\Yvet}_{cs}^{[m]} \; \widetilde{\Yvet}_{cs}^{[k_{p-1}]} \ldots \widetilde{\Yvet}_{cs}^{[k_2]} \; \widetilde{\Yvet}_{cs}^{[1]}
			\right] = \Mvet_{cs} \left[ \widehat{\Yvet}^{[m]} \; \widehat{\Yvet}^{[k_{p-1}]} \ldots \widehat{\Yvet}^{[k_2]} \; \widehat{\Yvet}^{[1]}
			\right] = \Mvet_{cs}\widehat{\Yvet}, \\
			\widetilde{\Yvet}_{te} & = & \left\{\Mvet_{te} \left[ \widehat{\yvet}_1 \ldots \widehat{\yvet}_i \ldots \widehat{\yvet}_n \right]\right\}' = \left\{\Mvet_{te}\widehat{\Yvet}'\right\}' .
		\end{array}
		$$
		
		Then, $\widetilde{\Yvet}_{cst}$ is obtained by first operating a cross-sectional reconciliation (step 1, $\widetilde{\Yvet}_{cs}$), and then reconciling via temporal hierarchies the forecasts obtained in the previous step (step 2, $\widetilde{\Yvet}_{cst}$). In matrix terms:
		$$
		\begin{array}{rcl}
			\text{step 1 } &
			\widetilde{\Yvet}_{cs} &= \Mvet_{cs}\widehat{\Yvet} \\
			\text{step 2 } &
			\widetilde{\Yvet}_{cst} &= \left\{\Mvet_{te} \widetilde{\Yvet}_{cs}'\right\}' = \widetilde{\Yvet}_{cs}\Mvet_{te}' = \Mvet_{cs}\widehat{\Yvet}\Mvet_{te}'
		\end{array}
		$$
		where $\widehat{\Yvet}$ is the ($n\times (k^\ast+m)$) base forecasts matrix.
		Viceversa, $\widetilde{\Yvet}_{tcs}$ is obtained by first operating a temporal reconciliation (step 1, $\widetilde{\Yvet}_{te}$), and finally a cross-sectional reconciliation is applied (step 2):
		$$
		\begin{array}{rcl}
			\text{step 1 } & \widetilde{\Yvet}_{te} & = \left\{\Mvet_{te} \widehat{\Yvet}'\right\}' =\widehat{\Yvet}\Mvet_{te}'\\
			\text{step 2 } & \widetilde{\Yvet}_{tcs} & = \Mvet_{cs} \widetilde{\Yvet}_{te} =\Mvet_{cs} \widehat{\Yvet}\Mvet_{te}' = \widetilde{\Yvet}_{cst} .
		\end{array}
		$$
The forecasts $\widetilde{\Yvet}_{tcs}$ (and $\widetilde{\Yvet}_{cst}$) (a single two-step iteration) are cross-temporally reconciled because:
		$$
		\begin{aligned}
			\Uvet'\widetilde{\Yvet}_{tcs} &= \Uvet'\Mvet_{cs} \widehat{\Yvet}\Mvet_{te}'= \left[\Uvet' - \Uvet'\Wvet\Uvet\left(\Uvet'\Wvet\Uvet\right)^{-1}\Uvet'\right]  \widehat{\Yvet}\Mvet_{te}'=\left[\Uvet' - \Uvet'\right]  \widehat{\Yvet}\Mvet_{te}' = \Zerovet_{n_a \times (k^\ast+ m)}
		\end{aligned}
		$$
		and
		$$
		\begin{aligned}
			\Zvet'\widetilde{\Yvet}_{tcs}' &= \Zvet'\Mvet_{te} \widehat{\Yvet}'\Mvet_{cs}' = \left[\Zvet' - \Zvet'\Omegavet\Zvet\left(\Zvet'\Omegavet\Zvet\right)^{-1}\Zvet'\right] \Mvet_{cs}'=\left[\Zvet' - \Zvet'\right] \widehat{\Yvet}'\Mvet_{cs}'= \Zerovet_{m \times n}.
		\end{aligned}
		$$
		
		\item Using matrix vectorization and structural representation for the cross-temporal reconciliation problem we have: 
		$$
		\begin{aligned}
			\widetilde{\yvet}_{oct} = \Fvet \left(\Fvet' \Omegavet_{ct}^{-1}\Fvet\right)^{-1}\Fvet'\widehat{\yvet}
		\end{aligned} ,
		$$
		where $\widetilde{\yvet}_{oct} = \mathrm{vec}\left(\widetilde{\Yvet}_{oct}'\right)$, $\widehat{\yvet} = \mathrm{vec}\left(\widehat{\Yvet}_{oct}'\right)$, %$\Svet$ is the ($n\times n_b$) cross-sectional summing matrix, $\Rvet$ is the [$(k^\ast +m)\times m$] temporal summing matrix and 
		and $\Fvet = \Svet \otimes \Rvet$ is the [$n(k^\ast +m)\times mn_b$] cross-temporal summing matrix. Let $\Omegavet_{ct} = \Wvet \otimes \Omegavet$ be the cross-temporal error covariance matrix, by exploiting the properties of the Kronecker product (\citealp{Henderson1981}; \citealp{Harville2008}), we obtain:
%		Kronecker's product has the following properties (\citealp{Harville2008}):
%		\begin{itemize}
%			\item transpose property, $(\Avet\otimes \Bvet)' = \Avet' \otimes \Bvet'$;
%			\item inverse property, $(\Avet\otimes \Bvet)^{-1} = \Avet^{-1} \otimes \Bvet^{-1}$;
%			\item mixed-product property, $(\Avet\otimes \Bvet)(\Cvet\otimes \Dvet) = (\Avet\Cvet\otimes \Bvet\Dvet)$.
%		\end{itemize}
%		In addition, we have also the non-commutative property (\citealp{henderson1981}): $(\Bvet \otimes \Avet) = \Pvet (\Avet\otimes \Bvet) \Pvet'$ where $\Pvet$ is the permutation matrix.
%		Now let $\Omegavet_{ct} = \Wvet \otimes \Omegavet$, then:
		$$
		\begin{aligned}
			\widetilde{\yvet}_{oct} &= \Fvet \left(\Fvet' \Omegavet_{ct}^{-1}\Fvet\right)^{-1}\Fvet'\Omegavet_{ct}^{-1}\widehat{\yvet} \\
			&= (\Svet \otimes \Rvet)\left[(\Svet \otimes \Rvet)' (\Wvet \otimes \Omegavet)^{-1} (\Svet \otimes \Rvet)\right]^{-1}(\Svet \otimes \Rvet)'(\Wvet \otimes \Omegavet)^{-1}\widehat{\yvet}\\
			& = (\Svet \otimes \Rvet)\left[(\Svet' \otimes \Rvet') (\Wvet^{-1}  \otimes \Omegavet^{-1} )(\Svet \otimes \Rvet)\right]^{-1}(\Svet' \otimes \Rvet')(\Wvet^{-1} \otimes \Omegavet^{-1})\widehat{\yvet}\\
			& = (\Svet \otimes \Rvet)\left(\Svet'\Wvet^{-1}\Svet \otimes \Rvet'\Omegavet^{-1}\Rvet\right)^{-1}(\Svet'\Wvet^{-1} \otimes \Rvet'\Omegavet^{-1})\widehat{\yvet}\\
			& = \left[\Svet\left(\Svet'\Wvet^{-1}\Svet\right)^{-1}\Svet'\Wvet^{-1} \otimes \Rvet\left(\Rvet'\Omegavet^{-1}\Rvet\right)^{-1}\Rvet'\Omegavet^{-1}\right]\widehat{\yvet}.
		\end{aligned}
		$$
		Exploiting the structural notation also in the \textit{temporal then cross-sectional} iterative procedure and the vectorization $\widetilde{\yvet}_{tcs} = \mathrm{vec}\left(\widehat{\Yvet}_{tcs}'\right)$, we obtain:
		$$
		\begin{aligned}
			\widetilde{\yvet}_{tcs} &= \Pvet \left[\Ivet_{k^\ast + m} \otimes \Svet\left(\Svet'\Wvet^{-1}\Svet\right)^{-1}\Svet'\Wvet^{-1}\right] \Pvet' \left[\Ivet_{n} \otimes \Rvet \left(\Rvet'\Omegavet^{-1}\Rvet\right)^{-1}\Rvet'\Omegavet^{-1}\right]\widehat{\yvet}\\
			&= \left[\Svet\left(\Svet'\Wvet^{-1}\Svet\right)^{-1}\Svet'\Wvet^{-1} \otimes \Ivet_{k^\ast + m}\right] \left[\Ivet_{n} \otimes \Rvet \left(\Rvet'\Omegavet^{-1}\Rvet\right)^{-1}\Rvet'\Omegavet^{-1}\right]\widehat{\yvet} \\
			&=\left[\Svet\left(\Svet'\Wvet^{-1}\Svet\right)^{-1}\Svet'\Wvet^{-1} \otimes \Rvet \left(\Rvet'\Omegavet^{-1}\Rvet\right)^{-1}\Rvet'\Omegavet^{-1}\right]\widehat{\yvet} = \widetilde{\yvet}_{oct}.
		\end{aligned}
		$$
		Finally, $\widetilde{\Yvet}_{tcs} = \widetilde{\Yvet}_{oct}$ and, following from point 1, $\widetilde{\Yvet}_{tcs} = \widetilde{\Yvet}_{cst} = \widetilde{\Yvet}_{oct}$.
	\end{enumerate}
\hfill $\Box$

\subsection*{The heuristic KA with constant cross-sectional and temporal error covariance matrices}
In the \cite{Kourentzes2019} procedure, the temporally reconciled predictions at step 1, $\widehat{\Yvet}\Mvet_t'$, are then cross-sectionally reconciled via premultiplication by the matrix $\overline{\Mvet} = \frac{1}{|\mathcal{K}|} \sum_{k \in \mathcal{K}} \Mvet^{[k]}_{cs}$ such that
$$
\widetilde{\Yvet}_{KA} = \overline{\Mvet}\widehat{\Yvet}\Mvet_t' = \frac{1}{|\mathcal{K}|} \sum_{k \in \mathcal{K}} \Mvet^{[k]}_{cs} \widehat{\Yvet}\Mvet_t' = \Mvet_{cs}\widehat{\Yvet}\Mvet_t' = \widetilde{\Yvet}_{tcs},
$$
where $\frac{1}{|\mathcal{K}|} \sum_{k \in \mathcal{K}} \Mvet^{[k]}_{cs} = \Mvet_{cs}$ because $\Mvet^{[k]}_{cs} = \Mvet_{cs}$ by assumption ($\Wvet^{[k]} = \Wvet$ for $k \in \mathcal{K}$).

\newpage

\section{Auxiliary tables}
\begin{center}
\begin{footnotesize}
\begin{longtable}{rllcccccc}
\caption{Number of series with at least one negative reconciled forecast.
		All temporal aggregation orders, forecast horizon: operating day.}
	\label{table_nn_Yagli_original_appendix} \\
\toprule
k & method & comb & type & n & min & max & fmin & fmax\\
\midrule
\endfirsthead

\multicolumn{9}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
k & method & comb & type & n & min & max & fmin & fmax\\
\midrule
\endhead

\bottomrule \multicolumn{9}{r}{{Continued on next page}} \\ 
\endfoot

\bottomrule
\endlastfoot

\input{./tab/table_nn_Yagli_original_appendix.tex}

\end{longtable}
\end{footnotesize}
\end{center}

%\begin{table}[H]
%	\caption{Number of replications with at least one negative reconciled forecast.
%		All temporal aggregation orders, forecast horizon: operating day.}
%	\label{table_nnrep_Yagli_original_appendix}
%	\begin{center}
%		\begin{footnotesize}
%			\input{table_nnrep_Yagli_original_appendix}
%		\end{footnotesize}
%	\end{center}
%\end{table}

\begin{center}
\begin{footnotesize}
\begin{longtable}{lllccccccccc}
	\caption{Number of replications with at least one negative reconciled forecast.
		All temporal aggregation orders, forecast horizon: operating day.}
	\label{table_nnrep_Yagli_original_appendix} \\

\toprule
$k$ & method & comb & type & \#L1 & \#L2 & \#L3 & \#tot & \%L1 & \%L2 & \%L3 & \%tot\\
\midrule
\endfirsthead

\multicolumn{12}{c}%
{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
\toprule
$k$ & method & comb & type & \#L1 & \#L2 & \#L3 & \#tot & \%L1 & \%L2 & \%L3 & \%tot\\
\midrule
\endhead

\bottomrule \multicolumn{12}{r}{{Continued on next page}} \\ 
\endfoot

\bottomrule
\endlastfoot

\input{./tab/table_nnrep_Yagli_original_appendix}

\end{longtable}	
\end{footnotesize}
\end{center}

\begin{figure}[H]
	\centering
	\includegraphics[width=0.9\linewidth]{img/comparison_PERS_vs_ct-struc_asp_0.pdf}
	\includegraphics[width=0.9\linewidth]{img/comparison_3TIER_vs_ct-struc_asp_0.pdf}
	\caption{Comparison of nRMSE(\%) between PERS$_{BU}$ and not negative oct-struc (top panel), and between 3TIER$_{BU}$ and not negative oct-struc (bottom panel). The black line represents the bisector, where the nRMSE's for both approaches are equal. On the top-left (bottom-right) corner of each graph, the percentage of points above (below) the bisector is reported.}
	\label{fig:comparison_ct-struc_vs_PERS_3TIER}
\end{figure}

%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth]{MCB_L3_k1_Yagli_original.pdf}
%		\caption{MCB-Nemenyi test: $\mathcal{L}_2$ hourly forecasts (318 series), forecast horizon: operating day. Base and 3TIER approaches coincide, then Base approach is not reported.}
%	\label{fig:MCB_L3k1_Yagli_original}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth]{MCB_L1L2L3_k1_Yagli_original.pdf}
%	\caption{MCB-Nemenyi test: $\mathcal{L}_0, \mathcal{L}_1, \mathcal{L}_2$ hourly forecasts (324 series), forecast horizon: operating day.}
%	\label{fig:MCB_L1L2L3k1_Yagli_original}
%\end{figure}
%
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth]{MCB_L3_k24_Yagli_original.pdf}
%	\caption{MCB-Nemenyi test: $\mathcal{L}_2$ daily forecasts (318 series), forecast horizon: operating day.}
%	\label{fig:MCB_L3k24_Yagli_original}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.9\linewidth]{MCB_L1L2L3_k24_Yagli_original.pdf}
%	\caption{MCB-Nemenyi test: $\mathcal{L}_0, \mathcal{L}_1, \mathcal{L}_2$ daily forecasts (324 series), forecast horizon: operating day.}
%	\label{fig:MCB_L1L2L3k24_Yagli_original}
%\end{figure}





==> tab/table_nnrep_Yagli_original.tex <==
\begin{tabular}[t]{l|cccc|cccc}
\toprule
         & \multicolumn{4}{c|}{Hourly forecasts} & \multicolumn{4}{c}{Daily forecasts}\\
         \cmidrule(lr){2-5} \cmidrule(lr){6-9}
Approach & $\mathcal{L}_0$ & $\mathcal{L}_1$ & $\mathcal{L}_2$ & Tot. & $\mathcal{L}_0$ & $\mathcal{L}_1$ & $\mathcal{L}_2$ & Tot.\\[-0.5em]
         & (1)             & (5)             & (318)           & (324) & (1)             & (5)             & (318) & (324)\\  
\midrule
base$^+$            &  1     & 5       & 0       & 6        & 0     & 2      & 58        & 60\\[-0.5em]
                    &(100\%) & (100\%) & (0\%)   & (1.85\%) & (0\%) & (40\%) & (18.24\%) & (18.52\%)\\
ct-ols              & 1      & 5       & 318     & 324      & 0     & 1      & 134       & 135\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (42.14\%) & (41.67\%)\\
cs-ols + t-struc    & 1      & 5       & 318     & 324      & 0     & 1      & 72        & 73\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (22.64\%) & (22.53\%)\\
cs-struc + t-ols    & 1      & 5       & 318     & 324      & 0     & 1      & 47        & 48\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (14.78\%) & (14.81\%)\\
ct-struc            & 1      & 5       & 318     & 324      & 0     & 0      & 17        & 17\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (0\%)  & (5.35\%)  & (5.25\%)\\
t-ols$_2$ + cs-ols$^*$     & 1      & 5       & 318     & 324      & 0     & 1      & 121        & 122\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (38.05\%) & (37.65\%)\\
t-struc$_2$ + cs-ols$^*$   & 1      & 5       & 318     & 324      & 0     & 1      & 102        & 103\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (32.08\%) & (31.79\%)\\
t-ols$_2$ + cs-struc$^*$   & 1      & 5       & 318     & 324      & 0     & 1     & 80         & 81\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (25.16\%) & (25.00\%)\\
t-struc$_2$ + cs-struc$^*$ & 1      & 5       & 318     & 324      & 0     & 1     & 41         & 42\\[-0.5em]
                    &(100\%) & (100\%) & (100\%) & (100\%)  & (0\%) & (20\%) & (12.89\%) & (12.96\%)\\
\bottomrule
\multicolumn{9}{l}{$^+$ The approach produces spatial (cross-sectional) and temporal incoherent forecasts.}\\
%\multicolumn{6}{l}{\; \; incoherent forecasts.} \\
\multicolumn{9}{l}{$^*$ The approach produces temporal incoherent forecasts.}
%\begin{tabular}[t]{lllccccccccc}
%\toprule
%$k$ & method & comb & type & \#L1 & \#L2 & \#L3 & \#tot & \%L1 & \%L2 & \%L3 & \%tot\\
%\midrule
%1 & NA & base & $\widehat{\textbf{y}}$ & 1 & 5 & 0 & 6 & 100.00\% & 100.00\% & 0.00\% & 1.85\%\\
%1 & ct & ols & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (cst) & ols-struc & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (cst) & struc-ols & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ct & struc & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (tcs) & ols2-ols & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (tcs) & struc2-ols & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (tcs) & ols2-struc & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%1 & ite (tcs) & struc2-struc & $\widetilde{\textbf{y}}$ & 1 & 5 & 318 & 324 & 100.00\% & 100.00\% & 100.00\% & 100.00\%\\
%\midrule
%24 & NA & base & $\widehat{\textbf{y}}$ & 0 & 2 & 58 & 60 & 0.00\% & 40.00\% & 18.24\% & 18.52\%\\
%24 & ct & ols & $\widetilde{\textbf{y}}$ & 0 & 1 & 134 & 135 & 0.00\% & 20.00\% & 42.14\% & 41.67\%\\
%24 & ite (cst) & ols-struc & $\widetilde{\textbf{y}}$ & 0 & 1 & 72 & 73 & 0.00\% & 20.00\% & 22.64\% & 22.53\%\\
%24 & ite (cst) & struc-ols & $\widetilde{\textbf{y}}$ & 0 & 1 & 47 & 48 & 0.00\% & 20.00\% & 14.78\% & 14.81\%\\
%24 & ct & struc & $\widetilde{\textbf{y}}$ & 0 & 0 & 17 & 17 & 0.00\% & 0.00\% & 5.35\% & 5.25\%\\
%24 & ite (tcs) & ols2-ols & $\widetilde{\textbf{y}}$ & 0 & 1 & 121 & 122 & 0.00\% & 20.00\% & 38.05\% & 37.65\%\\
%24 & ite (tcs) & struc2-ols & $\widetilde{\textbf{y}}$ & 0 & 1 & 102 & 103 & 0.00\% & 20.00\% & 32.08\% & 31.79\%\\
%24 & ite (tcs) & ols2-struc & $\widetilde{\textbf{y}}$ & 0 & 1 & 80 & 81 & 0.00\% & 20.00\% & 25.16\% & 25.00\%\\
%24 & ite (tcs) & struc2-struc & $\widetilde{\textbf{y}}$ & 0 & 1 & 41 & 42 & 0.00\% & 20.00\% & 12.89\% & 12.96\%\\
%\bottomrule
\end{tabular}


==> tex/cthier.tex <==
\begin{figure}[ht]
	\centering
	\resizebox{0.9\linewidth}{!}{
		\begin{tikzpicture}[baseline=(current  bounding  box.center),
	every node/.append style={shape=ellipse,
		draw=black},
	minimum width=1.2cm,
	minimum height=1.2cm]

	
	\node at (0, 0) (5Q1){$w^{[1]}_1$};
	\node at (1.5, 0) (5Q2){$w^{[1]}_2$};
	\node at (3, 0) (5Q3){$w^{[1]}_3$};
	\node at (4.5, 0) (5Q4){$w^{[1]}_4$};
	\node at (0.75, 1.8) (5SA1){$w^{[2]}_1$};
	\node at (3.75, 1.8) (5SA2){$w^{[2]}_2$};
	\node at (2.25, 3.6) (5A){$w^{[4]}_1$};
	\relation{0.2}{5Q1}{5SA1};
	\relation{0.2}{5Q2}{5SA1};
	\relation{0.2}{5Q3}{5SA2};
	\relation{0.2}{5Q4}{5SA2};
	\relation{0.2}{5SA1}{5A};
	\relation{0.2}{5SA2}{5A};
	\node[draw=none, align=center] at (0.25,3.6) {\Large $W$};
	
	\node at (11.5, 0) (6Q1){$z^{[1]}_1$};
	\node at (13, 0) (6Q2){$z^{[1]}_2$};
	\node at (14.5, 0) (6Q3){$z^{[1]}_3$};
	\node at (16, 0) (6Q4){$z^{[1]}_4$};
	\node at (12.25, 1.8) (6SA1){$z^{[2]}_1$};
	\node at (15.25, 1.8) (6SA2){$z^{[2]}_2$};
	\node at (13.75, 3.6) (6A){$z^{[4]}_1$};
	\relation{0.2}{6Q1}{6SA1};
	\relation{0.2}{6Q2}{6SA1};
	\relation{0.2}{6Q3}{6SA2};
	\relation{0.2}{6Q4}{6SA2};
	\relation{0.2}{6SA1}{6A};
	\relation{0.2}{6SA2}{6A};
	\node[draw=none, align=center] at (11.75,3.6) {\Large $Z$};
	
	\node at (5.75, 6.5) (7Q1){$x^{[1]}_1$};
	\node at (7.25, 6.5) (7Q2){$x^{[1]}_2$};
	\node at (8.75, 6.5) (7Q3){$x^{[1]}_3$};
	\node at (10.25, 6.5) (7Q4){$x^{[1]}_4$};
	\node at (6.5, 8.3) (7SA1){$x^{[2]}_1$};
	\node at (9.5, 8.3) (7SA2){$x^{[2]}_2$};
	\node at (8, 10.1) (7A){$x^{[4]}_1$};
	\relation{0.2}{7Q1}{7SA1};
	\relation{0.2}{7Q2}{7SA1};
	\relation{0.2}{7Q3}{7SA2};
	\relation{0.2}{7Q4}{7SA2};
	\relation{0.2}{7SA1}{7A};
	\relation{0.2}{7SA2}{7A};
	\node[draw=none, align=center] at (6,10.1) {\Large $X$};
	
%	\node[draw=black, fit={(1Q1) (1Q2) (1Q3) (1Q4) (1SA1) (1SA2) (1A)}](B1){};
%	\node[draw=black, fit={(2Q1) (2Q2) (2Q3) (2Q4) (2SA1) (2SA2) (2A)}](B2){};
%	\node[draw=black, fit={(3Q1) (3Q2) (3Q3) (3Q4) (3SA1) (3SA2) (3A)}](B3){};
%	\node[draw=black, fit={(4Q1) (4Q2) (4Q3) (4Q4) (4SA1) (4SA2) (4A)}](B4){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(5Q1) (5Q2) (5Q3) (5Q4) (5SA1) (5SA2) (5A)},
	minimum width=7cm,
	minimum height=5.5cm](U1){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(6Q1) (6Q2) (6Q3) (6Q4) (6SA1) (6SA2) (6A)},
	minimum width=7cm,
	minimum height=5.5cm](U2){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(7Q1) (7Q2) (7Q3) (7Q4) (7SA1) (7SA2) (7A)},
	minimum width=7cm,
	minimum height=5.5cm](T){};
%	\relation{0.3}{B1}{U1};
%	\relation{0.3}{B2}{U1};
%	\relation{0.3}{B3}{U2};
%	\relation{0.3}{B4}{U2};
	%\draw (T.south) -- +(0,-0.3) -| (U1.north)
	\relationDashed{0.3}{U1}{T};
	\relationDashed{0.3}{U2}{T};
	\end{tikzpicture}
	}
	\caption{Complete cross-temporal hierarchy for a quarterly two-level hierarchical time series.}
        \label{toyquarterlyhierarchy}
\end{figure}


==> tex/cthier_red.tex <==
\begin{figure}[ht]
	\centering
	\resizebox{0.9\linewidth}{!}{
		\begin{tikzpicture}[baseline=(current  bounding  box.center),
	every node/.append style={shape=ellipse,
		draw=black},
	minimum width=1.2cm,
	minimum height=1.2cm]

	
	\node at (0, 0) (5Q1){$w^{[1]}_1$};
	\node at (1.5, 0) (5Q2){$w^{[1]}_2$};
	\node at (3, 0) (5Q3){$w^{[1]}_3$};
	\node at (4.5, 0) (5Q4){$w^{[1]}_4$};
	\node at (2.25, 1.8) (5A){$w^{[4]}_1$};
	\relation{0.2}{5Q1}{5A};
	\relation{0.2}{5Q2}{5A};
	\relation{0.2}{5Q3}{5A};
	\relation{0.2}{5Q4}{5A};
	\node[draw=none, align=center] at (0.25,1.8) {\Large $W$};
	
	\node at (11.5, 0) (6Q1){$z^{[1]}_1$};
	\node at (13, 0) (6Q2){$z^{[1]}_2$};
	\node at (14.5, 0) (6Q3){$z^{[1]}_3$};
	\node at (16, 0) (6Q4){$z^{[1]}_4$};
	\node at (13.75, 1.8) (6A){$z^{[4]}_1$};
	\relation{0.2}{6Q1}{6A};
	\relation{0.2}{6Q2}{6A};
	\relation{0.2}{6Q3}{6A};
	\relation{0.2}{6Q4}{6A};
	\node[draw=none, align=center] at (11.75,1.8) {\Large $Z$};
	
	\node at (5.75, 4.5) (7Q1){$x^{[1]}_1$};
	\node at (7.25, 4.5) (7Q2){$x^{[1]}_2$};
	\node at (8.75, 4.5) (7Q3){$x^{[1]}_3$};
	\node at (10.25, 4.5) (7Q4){$x^{[1]}_4$};
	\node at (8, 6.3) (7A){$x^{[4]}_1$};
	\relation{0.2}{7Q1}{7A};
	\relation{0.2}{7Q2}{7A};
	\relation{0.2}{7Q3}{7A};
	\relation{0.2}{7Q4}{7A};
	\node[draw=none, align=center] at (6,6.3) {\Large $X$};
	
%	\node[draw=black, fit={(1Q1) (1Q2) (1Q3) (1Q4) (1SA1) (1SA2) (1A)}](B1){};
%	\node[draw=black, fit={(2Q1) (2Q2) (2Q3) (2Q4) (2SA1) (2SA2) (2A)}](B2){};
%	\node[draw=black, fit={(3Q1) (3Q2) (3Q3) (3Q4) (3SA1) (3SA2) (3A)}](B3){};
%	\node[draw=black, fit={(4Q1) (4Q2) (4Q3) (4Q4) (4SA1) (4SA2) (4A)}](B4){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(5Q1) (5Q2) (5Q3) (5Q4) (5A)},
	minimum width=7cm,
	minimum height=3.5cm](U1){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(6Q1) (6Q2) (6Q3) (6Q4) (6A)},
	minimum width=7cm,
	minimum height=3.5cm](U2){};
	\node[draw=black, shape=rectangle, dashed, line width=0.3mm, fit={(7Q1) (7Q2) (7Q3) (7Q4) (7A)},
	minimum width=7cm,
	minimum height=3.5cm](T){};
%	\relation{0.3}{B1}{U1};
%	\relation{0.3}{B2}{U1};
%	\relation{0.3}{B3}{U2};
%	\relation{0.3}{B4}{U2};
	%\draw (T.south) -- +(0,-0.3) -| (U1.north)
	\relationDashed{0.3}{U1}{T};
	\relationDashed{0.3}{U2}{T};
	\end{tikzpicture}
	}
	\caption{Reduced cross-temporal hierarchy for a quarterly two-level hierarchical time series.}
        \label{toyquarterlyhierarchy_red}
\end{figure}


==> tex/estratti.tex <==
\section{Estratti da paper}

\textbf{\cite{Yagli2019}}

Photovoltaic (PV) generation has a stochastic nature and is related to weather variables such as temperature, water vapor, aerosol levels, and in particular, cloud movements. Because of the variable generation, PV-generated power introduces broad challenges to the utility grid operators. These challenges include congestion and reliability issues due to fluctuation in PV generation, and inaccurate generation forecasts (Rickerson et al., 2014). To mitigate the effects of these issues, PV  output forecasting is required in various spatial scales and time horizons. Accurate forecasts are crucial for improving system reliability, generator scheduling, and planning of maintenance operations. Additionally, a recent study conducted by Martínez-Anido et al. (2013) showed the importance of forecasting and concluded that a 25\% improvement in PV output forecast accuracy can lead to 1.56\% (\$ 46.5 million) net reduction in generation cost in the simulated system.

The authors simulated the independent system operator (ISO) New England system using the PLEXOS production-cost modeling environment (Exemplar, 2013). In the simulation, a 25\% solar penetration (27,648 MW solar capacity) was assumed, and forecast horizon was 4 h. Whereas many solar forecasting methods have been proposed in the literature—see Yang et al. (2018) for a comprehensive review, conducted through text mining—the hierarchical nature of power generation is rarely considered during forecasting. In a power grid, PV-generated power can be modeled as a geographical hierarchy that consists of different levels such as inverter, PV plant, transmission zone (TZ), or interconnection operated by an ISO (this layer is referred to as ISO hereafter), see Fig. 1. Forecasts are required at all of these levels. From an ISO’s perspective, there are two ways to obtain solar forecasts: (1) forecast the overall solar generation directly, and (2) based on the (forecast generation) bids of individual power plant owners, and perform an aggregation (i.e., sum) of these individual forecasts. However, these two approaches are very unlikely to result in the same forecast, simply because the information and models used to generate the forecasts are different. This is known as aggregation inconsistency in space. A recent paper by Yang et al. (2017a) has addressed this issue by considering a so-called “geographical reconciliation” method. Through reconciliation, the forecasts obtained across a geographical hierarchy can be unified, i.e., become aggregate consistent.

Another type of aggregation inconsistency is related to forecast horizon and forecast resolution. For example, in the California ISO (CAISO) real-time market, 1-h-ahead forecasts need to be submitted in intervals of 5 min. In other words, twelve 5-min forecasts are required. These twelve forecasts can be generated in a variety of ways, e.g., (1) 12-step-ahead 
forecasting using 5-min data, (2) 6-step-ahead forecasting using 10-min data, and (3) 1-step-ahead forecasting using hourly data.1 With no surprise, these forecasts do not sum up; this is known as aggregation inconsistency in time. Such issue was addressed in another recent paper by \cite{Yang2017te}. The reconciliation method therein proposed is similar to the geographical reconciliation, but is carried out through a temporal hierarchy, see \cite{Yang2017te} for a graphical illustration.

Besides making the forecast aggregate-consistent, reconciling solar forecasts also improves accuracy. Since all forecasting models are associated with modeling error, by performing forecasting with different datasets (information) and models, the modeling error can be reduced. This concept is well-known by the name of “ensemble forecasting.” The fundamental concept in ensemble forecasting is to diversify the forecasts through segregating and perturbing the data and parameters (Yang and Dong, 2018; Yagli et al., 2018), and both above-mentioned reconciliation methods are essentially doing that. The geographical and temporal reconciliation methods have been shown promising in terms of generating aggregate-consistent forecasts and improving forecast accuracy. However, since the reconciliations are carried out in spatial and temporal domains separately, these reconciled forecasts can be further reconciled. Hence, this paper considers a method called “sequential reconciliation,” which reconciles the forecasts firstly in space then in time, or alternatively, firstly in time then in space. In this way, all forecasts in a spatio-temporal hierarchy are reconciled twice, presumably more accurate, and thus further benefit the ISOs, as well as other players in a power grid.

The remaining part of the paper is organized as follows. The forecast reconciliation framework is recapped in Section 2, whereas Section 3 describes the dataset and operational requirements. Section 4 describes sequential reconciliation approaches. Section 5 contains results and discussion. Conclusions follow at the end.

\textbf{\cite{Spiliotis2020b}}

Achieving high accuracy in load forecasting requires the selection of appropriate forecasting models, able to capture the special characteristics of energy consumption time series. When hierarchies of load from different sources are considered together, the complexity increases further; for example, when forecasting both at system and region level. Not only the model selection problem is expanded to multiple time series, but we also require aggregation consistency of the forecasts across levels. Although hierarchical forecast can address the aggregation consistency concerns, it does not resolve the model selection uncertainty. To address this we rely on Multiple Temporal Aggregation, which has been shown to mitigate the model selection problem for low frequency time series. We propose a modification for high frequency time series and combine conventional cross-sectional hierarchical forecasting with multiple temporal aggregation. The effect of incorporating temporal aggregation in hierarchical forecasting is empirically assessed using a real data set from five bank branches, demonstrating superior accuracy, aggregation consistency and reliable automatic forecasting.

Energy consumption forecasting encompasses a wide range of
forecasting problems. Achieving high forecast accuracy can yield significant improvements to energy management, leading to many economic and environmental benefits through energy conservation techniques such as load shifting, peak shaving, and energy-storing [1–3].
Moreover, it is crucial for maintaining the balance between the load and generation [4], as well as for planning the expansion of power grids [5]. Motivated by these potential gains, substantial work has been done
to improve energy forecasting methods and models, including statistical [6,7], machine learning [8], deep learning [9–11], and hybrid [12,13] approaches among others. Additionally, different methods exist according to the forecasting horizon considered, given that different decisions are supported per case [14].
The literature focuses on three main classes of methods based on the
prediction models used: statistical, engineering, and artificial intelligence methods. Suganthi and Samuel [15] provide a review of these
methods, while Zhao and Magoulès [16] focus on those used in the
building sector. They find that each forecasting method has its strengths
and weaknesses concerning the problem at hand, available data, and
the level of acceptable complexity. The literature does not identify the
best method, and therefore, the model selection problem remains an
unresolved key modeling issue [17]. This is particularly relevant in
practice, where a reliable selection of forecasts is desirable.
To mitigate this problem, in the general time series forecasting context, Kourentzes et al. [18] proposed using Multiple Temporal Aggregation (MTA), later generalized by [19]. This approach is based on temporally aggregating a time series at multiple levels, which transforms the
original data to lower time frequencies, highlighting different aspects of
the series [20]. Mainstream time series modeling literature has mainly
focused on identifying the single optimal level that makes modeling
simpler [21]. On the other hand, MTA models the series at multiple
aggregation levels and combines the resulting forecasts. This has two key
advantages: it provides a holistic modeling approach, focusing at both
high- and low-frequency components that are highlighted at different
temporal aggregation levels; and it mitigates modeling uncertainty, since
the final forecast is not based on a single forecasting model.
Mitigating modeling uncertainty is crucial when dealing with hierarchies and forecasting several connected time series. In most problems
related to energy conservation, management, and pricing, any decision
taken is multi-layered, considering and affecting multiple levels of the
energy system it refers to [22,23]. For example, when optimizing the
energy use of a building (top-level), the individual energy uses (heating,
cooling, lighting, etc.) must also be taken into consideration (bottom
level). These decisions are usually supported by forecasting systems,
which produce forecasts for all levels of the hierarchy. On the one hand,
this requires model selection and estimation for many time series and it
has the undesirable consequence that lower-level forecasts may not sum
up to the higher level forecasts and vice versa, as they are produced by
independent forecasting models. Forecasts, in this case, need to be
reconciled to ensure aggregation consistency across levels, as otherwise
decisions taken at different levels will not be aligned. To this end, cross-sectional hierarchical forecasting methods, such as “bottom-up” and “top-down”, have been proposed to achieve reconciliation [24].
Given the need for applying cross-sectional approaches to the problem at hand, the question arises whether MTA could be exploited to mitigate modeling uncertainty and improve forecasting performance, in a similar fashion to what has been reported in the literature for low-frequency time series forecasting problems. This is realized using the Multiple Aggregation Prediction Algorithm (MAPA) by Kourentzes et al. [18]. We propose a modification to make MAPA appropriate for high-frequency time series, i.e., better handling the undesirable effect of seasonality shrinkage that typical MTA approaches imply [25], and introduce an approach to combine conventional cross-sectional hierarchical forecasting with MAPA. Our results show that our approach
contributes towards (a) decreasing model uncertainty and increasing accuracy while (b) ensuring reconciled forecasts across the hierarchy.
Both enable automation of forecasting in such problems, aiding decision-makers. Based on the above, our contribution to the literature is twofold: (i) we evaluate the beneficial effect of cross-temporal aggregation in electricity consumption forecasting, and (ii) we provide an approach for effectively applying MTA to seasonal time series. The rest of the paper is organized as follows: in the next section, we review the work done so far in the temporal and cross-sectional aggregation literature. Section 3 describes our methodological approach, including the methods used. The data of our case study and the experimental set-up is presented in Section 4. Section 5 summarizes the results, followed by concluding remarks in Section 6.



%A hierarchical/grouped time series is a linearly constrained multiple time series consisting of a collection of time series that follows a hierarchical aggregation structure (\citealp{Panagiotelis2020a}).
%As an example, sales data can be disaggregated by product categories, and then by product subcategories, down to Stock Keeping Unit (SKU). In order to provide the appropriate demand forecast information given various managerial levels and functional disciplines within organizations, reliance on hierarchical forecasting is increasing, with the objective of producing coherent forecasts while improving their accuracy and reducing the overall forecasting burden (\citealp{Fliedner2001}).

%More generally, hierarchical/grouping forecasting is the process of generating coherent forecasts (or reconciling incoherent forecasts), allowing time series to be forecast individually, but preserving the relationships within the hierarchy/group (\citealp{Hyndman2021book}, ch. 11).
%It can be seen as a statistical device that can improve forecast accuracy through the use of forecast combination, whose main motivation is to provide coherent predictions for decisions at different levels of the hierarchy.

%Classical reconciliation approaches are bottom-up, top-down, and middle-out (\citealp{Athanasopoulos2009}).
%Bottom-up forecasting (\citealp{Dunn1976}) involves forecasting the most granular level of the hierarchy, then aggregating up to create estimates for the higher levels. The main advantage of this method is that, because forecasts are obtained at the lowest level of the hierarchy, no information is lost due to aggregation. However, it ignores the relationships between the series, and usually performs poorly on highly aggregated data. Furthermore, information at lower levels of the hierarchy tends to be noiser, potentially resulting in a reduced overall forecast accuracy.
%In the top-down approach (\citealp{Gross1990}), the top level of the hierarchy is first forecast, and then this forecast is split up to get estimates for the lower levels, typically using historical or forecasted proportions (\citealp{Athanasopoulos2009}).
%The middle-out approach is a combination of the bottom-up and top-down approaches: the middle level (neither the most granular nor the most aggregated) variables are forecast. These values are then used to compute the higher levels' forecasts using the bottom-up approach, and the lower levels with the top-down approach.
%
%Modern least squares-based reconciliation techniques emerged in the cross-sectional framework (optimal combination approach, \citealp{Hyndman2011}), and have then been extended both in temporal (\citealp{Athanasopoulos2017}, \citealp{Nystrup2020}), and cross-temporal (\citealp{Kourentzes2019}, \citealp{DiFonzoGiro2021}) frameworks, designed to align short- and long-term forecasts for consistency of different planning and budgeting purposes. %, possibly to effectively get a coherent one-number-forecast.
%This class of techniques is usually associated to a forecasting scheme where all the time series are independently forecast at all levels (cross-sectional and/or temporal), producing incoherent base forecasts, that are then transformed using all the information and relationships a hierarchy can offer in order to be coherent along the chosen dimensions (cross-sectional, temporal, or both). This result is obtained using a linear regression model, and the newly coherent forecasts are a weighted sum of the forecasts from all levels, with the weights found by solving a system of equations ensuring the natural relationships between the different levels of the hierarchy are satisfied.
%If the base forecasts are unbiased, \cite{Hyndman2011} show that the optimal combination approach provides unbiased reconciled forecasts at all levels with minimal loss of information, taking advantage of the relationships between time series to find patterns. 
%
%In practice, the best choice is oftentimes a combination of hierarchies, as forecast accuracy tends to improve if the model can learn from multiple relationships (\citealp{Bates1969}, \citealp{Timmermann2006}). Moving from this observation, 
%in a recent paper, while elucidating the links between forecast combination and cross-sectional forecast reconciliation, \cite{Hollyman2021} have proposed a forecast combination-based approach to the reconciliation of a simple hierarchy. A new Level Conditional Coherent ($LCC$) point forecast reconciliation procedure was developed, and it was shown that the simple average of a set of $LCC$, and bottom-up reconciled forecasts (called Combined Conditional Coherent, $CCC$) results in good performance as compared to those obtained through the state-of-the-art cross-sectional reconciliation procedures (\citealp{Wickramasuriya2019}). %(\citealp{Wickramasuriya2019}).
%In this paper, we build upon and extend this proposal along some new directions.
%\begin{enumerate}
%\item We shed light on the nature and the mathematical derivation of the $LCC$ reconciliation formula, showing that it is the result of an exogenously linearly constrained  minimization of a quadratic loss function in the differences between the target and the base forecasts with a diagonal associated matrix.
%\item Endogenous constraints may be considered as well, resulting in level conditional reconciled forecasts of all the involved series, where both the upper and the bottom time series are coherently revised.
%We show that even in this framework it is still valid the interesting interpretation given by \cite{Hollyman2021} of the reconciliation formula as the combination of direct (base) and indirect forecasts, the latter ones depending on the accounting relationships linking upper and bottom series.
%The extension to the cases where a full metric matrix is considered in the definition of the loss function is straightforward, which might be useful when (if) suitable error forecast covariance matrices may be estimated.
%\item We show that the $LCC$ approach (i.e., with exogenous constraints, but the result holds in the endogenous case as well) does not guarantee the non-negativity of the reconciled forecasts. Thus we argue that - when the variables to be forecast are intrinsically non-negative - interpreting $LCC$ as an `unbiased top-down reconciliation procedure' (\citealp{Hollyman2021}) leaves room for some doubts. 
%%In this latter case, possible non-negativity issues in the reconciled forecasts are appropriately dealt with.
%%Then, in order to exploit the inherent relationships valid for a hierarchy/group of time series to achieve better forecast accuracy, we extend the $LCC$ (and $CCC$ as well) forecast reconciliation procedures both in the temporal and cross-temporal frameworks.
%\item The new procedures, available in the \texttt{R} package \texttt{FoReco} (\citealp{FoReco2021}), 
%are used in a forecasting experiment on the classical Australian Tourism Demand (Visitor Nights) dataset, where the original results found by \cite{Hollyman2021} are re-assessed (i) using the relative accuracy indices for multiple comparisons recommended by \cite{Davydenko2013}, and (ii) taking into account the non-negativity issues posed by the dataset at hand.
%\item Finally, due to the crucial role played by the (possibly different) models used to compute the base forecasts, the $CCC$ reconciliation strategy proposed by \cite{Hollyman2021} (called $CCC_H$ in our paper) is interpreted as a forecast pooling strategy (\citealp{Hendry2004}, \citealp{Marcellino2004}, \citealp{Geweke2011}, \citealp{KourentzesBarrowPetropoulos2019}), 
%%well performing as compared to the state-of-the-art cross-sectional forecast reconciliation approaches (\citealp{Wickramasuriya2019}).
%and we show that the intuition behind the $CCC_H$ strategy can be further improved by adopting a somehow less arbitrary simple forecast averaging strategy.
%\end{enumerate}
%
%
%The paper is organized as follows. In section \ref{sec:notation} we set the notation, define the forecast reconciliation problem, and show the Level Conditional Coherent forecast reconciliation approach proposed by \cite{Hollyman2021}.
%We re-interpret this procedure in terms of an optimization problem, with either exogenous (section \ref{sec:LCCexo}), or endogenous (section \ref{sec:LCCendo}) constraints, which encompasses the forecast reconciliation procedure so far as a particular case.
%An empirical application is performed in section \ref{sec:VN525}, where the rolling forecast experiment performed by \cite{Hollyman2021} is reprised and extended in light of the new insights.
%Section \ref{sec: conclusions} contains conclusions and indications for future research. An on-line appendix contains supplementary tables and graphs related to the empirical application. 
 

